XNect: Real-time Multi-Person 3D Motion Capture with a Single RGB Camera

We present a real-time approach for multi-person 3D motion capture at over 30 fps using a single RGB camera. It operates successfully in generic scenes which may contain occlusions by objects and by other people. Our method operates in subsequent stages. The first stage is a convolutional neural network (CNN) that estimates 2D and 3D pose features along with identity assignments for all visible joints of all individuals.We contribute a new architecture for this CNN, called SelecSLS Net, that uses novel selective long and short range skip connections to improve the information flow allowing for a drastically faster network without compromising accuracy. In the second stage, a fully connected neural network turns the possibly partial (on account of occlusion) 2Dpose and 3Dpose features for each subject into a complete 3Dpose estimate per individual. The third stage applies space-time skeletal model fitting to the predicted 2D and 3D pose per subject to further reconcile the 2D and 3D pose, and enforce temporal coherence. Our method returns the full skeletal pose in joint angles for each subject. This is a further key distinction from previous work that do not produce joint angle results of a coherent skeleton in real time for multi-person scenes. The proposed system runs on consumer hardware at a previously unseen speed of more than 30 fps given 512x320 images as input while achieving state-of-the-art accuracy, which we will demonstrate on a range of challenging real-world scenes.

==> Tables/mupots_input_ablation.tex <==
%%!TEX root = ../article.tex
\renewcommand{\tabcolsep}{2.0pt}
%\begin{table}[]
\centering
\caption{Evaluation of choices for input to the 2nd stage on MuPoTS. The metric used is 3D percentage of correct keypoints (\textbf{PCK}), so higher is better. The data set contains 20 test scenes \textbf{T1-T20}. We evaluate once on all annotated poses (top row - \textbf{All}),
Evaluation of the impact of the different components from \textit{Stage I} that form the input to \textit{Stage II}, evaluated on the multi person 3D pose benchmark MuPoTS-3D~\cite{mehta_3dv18}. We evaluate on all annotated subjects using the 3D percentage of correct keypoints (\textbf{3DPCK}) metric, also showing the accuracy split for visible and occluded joints. The components evaluated are the 2D pose predictions $P_{k}^{2D}$, the body joint confidences $C_k$, and the set of extracted 3D features $\{l_{j,k}\}_{j=1}^{J}$. 
}
%\label{tbl:coco_eval}

%\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|c|c}
\textbf{Stage II}    & \multicolumn{4}{c}{\textbf{3DPCK}}                 \\
\textbf{Input}       & \textbf{~~~All~~~} & \textbf{~~~Matched~~~} &\textbf{Visible} & \textbf{Occluded} \\ \hline
$P_{k}^{2D}$              \T    & 59.3         & 63.9             & 61.6 & 50.0              \\
$P_{k}^{2D} + C_k$          \T   & 64.1         & 69.1             & 67.6  &  51.7          \\
$P_{k}^{2D} + C_k + \{l_{j,k}\}_{j=1}^{J} $\T        & 70.4         & 75.8             & 74.1  & 57.8              \\
\end{tabular}
%} 
